A Pedestrian Detection and Tracking Framework for Autonomous Cars: Efficient Fusion of Camera and LiDAR Data

This paper presents a novel method for pedestrian detection and tracking by fusing camera and LiDAR sensor data. To deal with the challenges associated with the autonomous driving scenarios, an integrated tracking and detection framework is proposed. The detection phase is performed by converting LiDAR streams to computationally tractable depth images, and then, a deep neural network is developed to identify pedestrian candidates both in RGB and depth images. To provide accurate information, the detection phase is further enhanced by fusing multi-modal sensor information using the Kalman filter. The tracking phase is a combination of the Kalman filter prediction and an optical flow algorithm to track multiple pedestrians in a scene. We evaluate our framework on a real public driving dataset. Experimental results demonstrate that the proposed method achieves significant performance improvement over a baseline method that solely uses image-based pedestrian detection.

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/config/packages.tex <==
\usepackage{multicol}
\usepackage[bookmarks=true]{hyperref}
\usepackage{cite}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{pgfplots}
\usepackage{tikz}
\usepackage{subcaption}
\usepackage{hyperref}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{float}
\usepackage{todonotes}
\usepackage{amsmath}
\DeclareMathOperator*{\argmax}{argmax}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\colorlet{negro}{black}
\colorlet{gris}{black!70}
\colorlet{rojo}{red!70!black}
\colorlet{rojol}{red}
\usepackage{booktabs}
\usepackage{color, colortbl}
\definecolor{Gray}{gray}{0.9}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\newcolumntype{b}{>{\columncolor{white}}c}
\usepackage{epstopdf}
\newcommand{\ts}{\textsuperscript}


==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/config/packages_old.tex <==

%% Added Package
% amsmath and amssymb packages, useful for mathematical formulas and symbols
\usepackage{amsmath,amssymb,graphicx,breqn}
% for adding definition in writing
\usepackage{amsfonts,amsthm,epsfig,epstopdf,titling,url,array}

% cite package, to clean up citations in the main text. Do not remove.
\usepackage[noadjust]{cite} % for [] - [] citation
% \usepackage[sort&compress]{cite}
\bibliographystyle{ieeetr} % From outside Calling
% Use nameref to cite supporting information files (see Supporting Information section for more info)
\usepackage{url,nameref}
%\usepackage[hidelinks=true]{hyperref} % For Referencing without box
\usepackage{hyperref} % For Referencing but red box
% \usepackage[hidelinks=true]{hyperref} % For Referencing

\usepackage{setspace} % for controlling spacing in line
\usepackage{color}
\usepackage{ragged2e} % For Justification

% color can be used to apply background shading to table cells only
\usepackage[table]{xcolor}

% for adding definition in writing
\theoremstyle{plain}
\newtheorem{thm}{Theorem}%[section]
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem*{cor}{Corollary}

\theoremstyle{definition}
\newtheorem{defn}{Definition}%[section]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{exmp}{Example}%[section]

\newtheorem{rem}{Remark}%[section]

\theoremstyle{remark}
%\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}


% Figure Purpose
\usepackage{graphicx}
\usepackage{subcaption}

% For Caption Legend adding purpose
\usepackage{color}
\usepackage{tikz}
\usetikzlibrary{shapes}

%In case you encounter the following error:
%Error 1010 The PDF file may be corrupt (unable to open PDF file) OR
%Error 1000 An error occurred while parsing a contents stream. Unable to analyze the PDF file.
%This is a known problem with pdfLaTeX conversion filter. The file cannot be opened with acrobat reader
%Please use one of the alternatives below to circumvent this error by uncommenting one or the other
%\pdfobjcompresslevel=0
%\pdfminorversion=4

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document

% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%\usepackage{amsmath} % assumes amsmath package installed
%\usepackage{amssymb}  % assumes amsmath package installed



==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/architecture.tex <==
%% Creator: Inkscape inkscape 0.92.4, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'architectureGradient.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To Scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{309.64281878bp}%
    \ifx\svgScale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgScale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgScale\undefined%
  \makeatother%
  \begin{picture}(1,1.10224947)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength]{figtex/architecture.eps}}%
   \put(0.163438817,0.2005536){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Conv\end{tabular}}}}%
    \put(0.0922034,0.44100306){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Average Pooling\end{tabular}}}}%
    \put(0.0922034,0.68204425){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Average Pooling\end{tabular}}}}%
    \put(0.0922034,0.92760688){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Average Pooling\end{tabular}}}}%
    
    %%%standard
    \put(0.07922034,0.31941654){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1\ts{st} Scale Feature Map\end{tabular}}}}%
    \put(0.07922034,0.56290941){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}2\ts{nd} Scale Feature Map\end{tabular}}}}%
    \put(0.07922034,0.80290707){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}3\ts{rd} Scale Feature Map\end{tabular}}}}%
    \put(0.07922034,1.04812196){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}4\ts{th} Scale Feature Map\end{tabular}}}}%
    
    
    \put(0.595422909,0.67666367){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Shared\\ Tower\end{tabular}}}}%
    \put(0.863341397,0.79304843){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}  Box\\Score\end{tabular}}}}%
    \put(0.863341397,0.54578977){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}   Box\\Location\end{tabular}}}}%
    \put(0.122034,0.08006312){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Base Network\\(MobileNet)\end{tabular}}}}%
  
  \end{picture}%
\endgroup%


==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/classification.tex <==

% \begin{figure}[h!]
%     % \includegraphics[trim={0,0,0,2cm},clip,width=8.65cm]{mashuk/Images/Loss_function.png}
%     \includegraphics{mashuk/Images/Loss_function.png}
%     \caption{Losses during training, run across $42k$ epochs. The red, green and blue lines represent total loss, localization loss and classification loss, respectively. }
%     \label{fig:Loss_function}
%   \end{figure}
 
 
 \begin{figure}[h!]

\begin{tikzpicture}
\begin{axis}[
xlabel={Number of epochs},
ylabel = {Loss}
]
  
\addplot table [x=No. of steps, y=Classification loss, col sep=comma] {resources/graph.csv};

\addplot table [x=No. of steps, y=Localization loss, col sep=comma] {resources/graph.csv};

\addplot table [x=No. of steps, y=Total loss, col sep=comma] {resources/graph.csv};

\legend{Classification loss,Localization loss,Total loss};

\end{axis}
\end{tikzpicture}
    \caption{Losses during training, run across $42\times 10^3$ epochs. The red, green and blue lines represent total loss, localization loss and classification loss, respectively. }
    \label{fig:Loss_function}
  \end{figure}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/cnn.tex <==
\begin{figure}[h!]
    \centering
    \vspace{4mm}
  \includegraphics[width=8.65cm]{Images/Mobilentet_conv.jpg}
  \caption{Comparison of Mobilenet convolutional operation with traditional Convolutional Operation \cite{howard2017mobilenets}: (a) Traditional convolution, (b) depthwise convolution, and (c) point-wise convolution operations in the context of Depthwise Separable Convolution.}
  \label{fig:Comparison of Convolution}
\end{figure}


==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/miss_rate_fppi_curve.tex <==
\begin{figure}[htb]
    \centering
    \vspace{-5pt}
    \includegraphics[width= 9cm]{Figures/benchmark.png}
    \caption{\small{The comparison among Fused-YOLO, Fusion without applying Kalman Filter, and Baseline YOLOv5. Fused-YOLO model get the lowest miss rate of $33.435\%$ among others.}\small{The comparison among Fused-YOLO, Fusion without applying Kalman Filter, and Baseline YOLOv5. Fused-YOLO model get the lowest miss rate of $33.435\%$ among others.}}
    \label{fig:Miss_rate_vs_fppi}
    \vspace{-5pt}
\end{figure}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/miss_rate_fppi_curve2.tex <==
% \begin{figure}[htb]
%     \centering
%     \vspace{-5pt}
%     \includegraphics[width= 9cm]{Figures/benchmark.png}
%     \caption{\small{The comparison of Fused-YOLO with YOLOv5. Fused-YOLO model get a lower miss rate compare to YOLOv5 model.}}
%     \label{fig:Miss_rate_vs_fppi}
%     \vspace{-5pt}
% \end{figure}

\begin{figure}[htb]
\begin{tikzpicture}
\begin{axis}[
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    xlabel={FPPI},
    ylabel={Miss Rate},
    xmin=0, xmax=1,
    ymin=0, ymax=0.6,
    xtick={0.2, 0.4, 0.6, 0.8, 1.0},
    xticklabels={$10^{-3}$,$10^{-2}$, $10^{-1}$, $10^{0}$, $10^{1}$ },
    ytick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
    legend pos=north east,
    ]
\addplot [color=blue, line width=1.6pt] table [x=x, y=y, col sep=comma] {resources/Fused-Yolo.csv};
\addlegendentry{Fused-Yolo (33.435)\%}
\addplot [color=darkgray,dashed, line width=1.6pt] table [x=x, y=y, col sep=comma] {resources/Fusion without KF.csv};
\addlegendentry{Fusion without KF (38.602)\%}
\addplot[color=red,dashed, line width=1.6pt] table [x=x, y=y, col sep=comma] {resources/Baseline method.csv};
\addlegendentry{Baseline method (41.945)\%}
\end{axis}
\end{tikzpicture}
    \caption{\small{The comparison among Fused-YOLO, Fusion without applying Kalman Filter, and Baseline YOLOv5. Fused-YOLO model get the lowest miss rate of $33.435\%$ among others.}}
    \label{fig:Miss_rate_vs_fppi}
\end{figure}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/mobilnet.tex <==


% \begin{figure}[htb]
%   \includegraphics[width=8.65cm]{Images/SSD-Mobilenet.png}

%   \caption{Architecture of the SSD-Mobilenet Model \cite{jin2018pooling}.}
%   \label{fig:Structure of SSD-Mobilenet Model}
% \end{figure}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/performance_table.tex <==
\begin{table}[htb]
\centering
\begin{tabular}{@{}lllllll@{}}
\toprule
Model & FP & TP  & FN & Accuracy & Precision & Recall \\ \midrule
YOLOv5   & 12 & 105 & 75 & 0.546    & 0.897     & 0.583  \\
Fused-YOLO & 12 & 117 & 63 & 0.609    & 0.900      & 0.650   \\ \bottomrule
\end{tabular}
\caption{Evaluation Metrics}
\label{tab:evaluation_metrics}
\end{table}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/ssd-mobilenet.tex <==
%% Creator: Inkscape inkscape 0.92.4, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'ssd-mobilenet.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{280.54945319bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.29970606)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength]{figtex/ssd-mobilenet.eps}}%
    
    % scale feature map
    \put(0.05128073,0.1845645){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1\ts{st} Scale Feature Map\end{tabular}}}}%
    \put(0.05128073,0.46453721){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}m\ts{th} Scale Feature Map\end{tabular}}}}%
    \put(0.03,0.734292){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(m+1)\ts{th} Scale Feature Map\end{tabular}}}}%
    \put(0.05128073,1.16140364){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}N\ts{th} Scale Feature Map\end{tabular}}}}%
    
    % conv
    \put(0.179113,0.6091571){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Conv\end{tabular}}}}%
    \put(0.179113,1.0317062){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Conv\end{tabular}}}}%
    
    % tower
    \put(0.603256874,0.22543618){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1\ts{st}\\tower\end{tabular}}}}%
    \put(0.603256874,0.7915123){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}m\ts{th}\\tower\end{tabular}}}}%
    \put(0.603256874,0.51153959){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(m+1)\ts{th}\\tower\end{tabular}}}}%
    \put(0.603256874,1.19818794){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}N\ts{th}\\tower\end{tabular}}}}%
    
    % box location
    \put(0.85841522,0.12573624){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    \put(0.85841522,0.40775252){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    \put(0.85841522,0.70694323){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    \put(0.85841522,1.10340087){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    
    % box score
    \put(0.85841522,0.27900572){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    \put(0.85841522,0.56306556){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    \put(0.85841522,0.85325627){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    \put(0.85841522,1.24971395){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    
    % base net
    \put(0.1457859,0.10581671){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Base Network\\(MobileNet)\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/ssd.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics{Images/SSD_feature_map.jpg}
    \caption{SSD Feature-map operation layers \cite{liu2016ssd}: (a) Input image with ground truth boxes, (b) 8x8 feature map showing default boxes with different aspect ratios, and (c) 8x8 feature map showing default boxes with different aspect ratios.}
    \label{fig:SSD feature map}
  \end{figure}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/table_compare_normal_data_set.tex <==
  \begin{table}[h!]
   \caption{Result comparison between SSD-Mobilenet and proposed method for fully visible pedestrians}
    \label{table:Result comparison of visible dataset}
    \begin{center}
    \begin{tabular}{|c||c||c||c|}
    \hline
    Model name & Correct detection & Miss detection & Perc. correct\\
    \hline
    SSD-Mobilenet & 526 & 87 & 85.80 \\ % inserting body of the table
    \hline
    Proposed method & 594 & 19 & 96.9 \\
    \hline
    \end{tabular}
    \end{center}
\end{table}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/table_dataset.tex <==
\begin{table}[h!]
    \caption{Result comparison between SSD-Mobilenet and proposed method for occluded dataset}
    \label{table:Result comparison of occluded dataset}
    \begin{center}
    \begin{tabular}{|c||c||c||c|}
    \hline
    Model name & Correct detection & Miss detection & Perc. correct\\
    \hline
    SSD-Mobilenet & 292 & 330 & 46.94 \\ % inserting body of the table
    \hline
    Proposed method & 594 & 28 & 95.49 \\
    \hline
    \end{tabular}
    \end{center}
\end{table}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/table_result.tex <==
\begin{table}[h]
    \caption{Result analysis with some fixed frames}
    \label{table:Result comparison}
    \begin{center}
    \begin{tabular}{|c||c||c||c|}
    \hline
    Object types & No. of Objects & Correct & Incorrect\\
    \hline
    Head & 500 & 454 & 46 \\ % inserting body of the table
    \hline
    Hand & 500 & 441 & 59 \\
    \hline
    Leg & 470 & 438 & 32 \\ 
    \hline
    \end{tabular}
    \end{center}
    \end{table}
    

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/figtex/yolo_architecture.tex <==
\begin{figure*}
    \vspace{3pt}
    \centering
    \includegraphics[height=6cm]{Images/Yolo_Architecture.pdf}
    \caption{\small{\textbf{Architecture of YOLOv5:} YOLOv5 has four major sections. It starts with input then merges to the backbone for feature extraction. Feature information is enhanced in the neck section, and the output section produces a bounding box with confidence scores for a specific class of objects}}
    \label{fig:Architecture_of_Yolo}
    \vspace{-10pt}
\end{figure*}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/sect/algo.tex <==

% %While testing our autonomous car, we figured out that some existing models of pedestrian detectors such as SSD-Mobilenet and Faster R-CNN confuse actual pedestrian with pedestrian crossing signs. Those models are trained with robust data sets and detect the pedestrian symbol within the pedestrian crossing sign, due to which detector can not distinguish between actual pedestrian and pedestrian crossing signs, which creates problems in decision making for the autonomous car. To overcome this problem, we have created a scale specific model to detect only the objects with expected size and those are actual pedestrians. In machine vision, object detection is challenging in many aspects, such as training data set creates a huge impact on detection specification. The preferred size of the desired object can be tuned by the model architecture. Based on the idea of specific or some desired expected output object size, we have tuned one of the well-known models. SSD-Mobilenet-V1 has been used for up to 90 different types of objects. But, we have trained that modified model for pedestrian detection only.  As the depth of the model is reduced, it speeds up the trained model detection performances. %
% So far we have explained the architecture of our base network.
% In this section, we explain our proposed method for pedestrian detection based on partial body parts. 

% % This allows within deformed shapes and occluded conditions. \todo{Not a complete sentence, please rewrite it.}
% % The proposed method also does not get confused by detecting pedestrian-like objects (those that are not actual pedestrians) by classifying them as a pedestrian. \todo{How do you validate this?}

% \subsection{Scale Specific Pooling operation (SSPO)}
% \input{figtex/sspm.tex}
% % Inspired by SSD-Mobilenet and Pooling Pyramid Network (PPN),  this section describes our proposed Scale Specific Pooling (SSP) model.  One of the major changes in our proposed model compared to SSD-Mobilenet is the replacement of convolution between feature maps with average pooling layers and we have done this differently scaled average pooling based on expected object sizes and ground truth box sizes.
% %\textcolor{red}{Inspired by PPN, We have used a shared tower for predicting box scores and locations for different body parts types.} This section also describes the effect of feature extraction for different body parts of the pedestrian compares to full body pedestrians. \textcolor{red}{We have made our model less complex and specific object detection oriented.}

% Scale Specific Pooling operation starts after the Mobilenet base network. 
% When we cascade Mobilenet with proposed SSPM the main adventage is, the combination reduces the scale factors in the images. In SSPM, we add convolutional feature layers and pooling layers to the end of our base network. These layers in FPN reduce the size progressively at different scales. We use some specific scale sizes average pooling for extracting different scale feature maps based on our training data and expected object sizes in test images. The differently scaled average pooling feature maps that we have used in our model are sized of $2\times2$, $4 \times 4$, $8 \times 8$ and $16 \times 16$. We trained our network with the pedestrian full body along with three body parts, and these consist of four different label IDs for each category. Training with body parts helps the model to extract more precise information about pedestrians.
% % \todo[inline]{explain how to train}
% %In our test, we assume the expected distance of pedestrians from the car is around 10m to 50m. Hence, 

% In SSPM, each feature layers can absolutely produce a fixed set of prediction maps with the help of convolutional filter and average pooling operation. The output of SSPO is a set of bounding boxes which got deafult sizes with each cell from each feature map. 
% Figure \ref{fig:Scale Specific Pooling Model} shows the structure of our proposed model.
% % After extracting feature information from the image using the mobilenet, our model takes a convolutional operation for generating the $1^{st}$  scale feature map. Then having three successive average pooling operations, we will have $2^{nd}$, $3^{rd}$ and, $4^{th}$ feature map layers. These feature maps use a shared tower to generate their prediction information. In our case, these shared towers consist of the information of the full body and three different body parts captured in different feature maps. 

 
% %From the mobilenet We have replaced the convolution operation with average pooling for different feature map layers, we have avoided addition and multiplication operation involving in convolution operation. Hence, the complexity of our model is reduced. We have used some specific scale sizes average pooling for extracting different scale feature maps as our model is trained for detecting only three different body parts (head, hand, and leg) along with full body of pedestrian, whereas SSD-Mobilenet is trained for ninety different types of object detection \textcolor{red}{with lot of variation in sizes.} As in this paper we consider pedestrian detection from a autonomous car's perspective, we want to detect the pedestrian while they are not a long distance from the car and considered the object size should not that small. The expected distance of pedestrian from the car that we considered in our test is around 10m to 50m. Considering the size of expected pedestrian body parts, the four pooling feature maps that we have used in our model are sized of 2 $\times$ 2, 4 $\times$ 4, 8 $\times$ 8 and 16 $\times$ 16. While we have trained our model, we have to make sure that the ratio of our highest scaled average pooling sizes, should grater than the ratio of the input image to the minimum sized ground truth box. So, the minimum sized ground truth box should be smaller in size compared with the smallest default box. On the other hand, to avoid false detection with a very small-sized object, we have considered our highest pooled feature map as 16 $\times$ 16.

% \subsection{Shared Tower}
% %\textcolor{red}{We can see from the architecture of SSD-Mobilenet shown in Figure \ref{fig:Structure of SSD-Mobilenet Model}, that the box scores and box locations are calculated for different feature layers, whereas }
% Shared towers consist of the information of the full body and three different body parts captured in different feature maps. 
% It is connected with each feature map layers and consists of feature information of the same location with different feature maps.
% % (Figure \ref{fig:Scale Specific Pooling Model}), which is similar to PPN model.
% Then it combines differently scaled feature maps to predict the final box score and its corresponding location. Thus, the shared tower provides classified object's score and bounding box location comparing the classified object's scores and bounding boxes of different feature map's output.
% % \todo[inline]{please provide more information}
% % As we have used shared box predictor in our model, that avoid miscalibration of score prediction with different scale as in case of with SSD-Mobilent \cite{jin2018pooling}. 


% %To overcome the problem with occlusion handling and pose variation, in our pedestrian detection model we have considered using three different body parts along with full body and the model consists of four different label IDs for three different body parts and a full body. So, feature extraction is more precise in the case of body parts compared to full body feature extraction. \textcolor{red}{While we trained our model with pedestrian body parts, the model consists of more precise information of the three body parts compared to a pedestrian detection model with a single ID.} For example, in the case of full-body pedestrian detection with SSD-Mobilenet, we found the model sometimes failed to detect the pedestrian while there is not enough gap between legs and hands are not stretch enough from the body. On the other hand in a similar scenario, the model with part detection can at least detect some body parts, though it can not detect the full body \ref{fig:Compared result of two model_test_image_2}. Our proposed model can detect the body parts as the model has more feature information for body parts. We have also set different threshold value for different body parts and these threshold value act like an weights for final detection, 
% %%
% %\subsection{Scale Specific pooling Model Architecture}
% %The architecture of the scale-specific model is very similar to the Pooling Pyramid Network(PPN), which is another modification of SSD-Mobilenet-V1. However, in pedestrian detection, we expect the size of our objects should not that small which is considered in SSD-Mobilenet for 90 different types of object detection. Hence, instead of taking various scaling as used in the SSD-mobilenet, in our model, for creating different feature maps, we have taken three specific ratios. On the other hand, we take all of our bounding boxes in the training dataset to be more than 28x56 pixel size and hence we consider average pooling for the different scaling features.

% %\begin{figure}[h!]
%  % \includegraphics{Images/Images1.jpg}
%  % \caption{Structure of SSD-Mobilenet Model\cite{jin2018pooling}}
%  % \label{fig:Structure of SSD-Mobilenet Model}
% %\end{figure}
% %We can see from the architecture of SSD-Mobilenet-V1 Figure \ref{fig:Structure of SSD-Mobilenet Model}, that the box scores and box locations are calculated for different feature layers whereas in scale specific pooling model we have used the shared tower for differently scaled feature maps to get the finalized box score and box location as in the case of PPN \cite{jin2018pooling}. Using SSD-Mobilenet, for pedestrian detection, we have found that there is some false detection with small scale object detection. To avoid the confusion with these small size object detection, we have designed our model to work with some specific scale only. We got better results with the scale size of 10x10, 5x5, 3x3 and 1x1 shown in Figure \ref{fig:Scale Specific Pooling Model}. 
% %\begin{figure}[h!]
%  % \includegraphics[width=8.65cm]{Images/scale_s_pooling.jpg}
%  % \caption{Structure of Scale Specific Pooling Model}
%  % \label{fig:Scale Specific Pooling Model}
% %\end{figure}
% %Instead of using a full-body dataset, we have used the body parts dataset for pedestrian detection. In the case of an occluded pedestrian, the detector used for full-body detection is not able to detect the object often, whereas our model which is trained with body parts, can detect some visible parts of the body to provide an idea about the actual object. As we eliminate the low scaling feature map layer and use average pooling instead of max pooling, it provides us more accurate information in the output layer. Average pooling captures more information as compared to max pooling, while there is a drastic change in intensity levels within the image.  

% % \subsection{Addition of repulsion loss}
% % We add repulsion loss for different body parts and detect the body parts more accurately in a crowded scenario. RepBox Loss. For RepBox Loss, we experiment with a different smooth parameter , reported in the fourth line of Table 1. When setting  as 0, RepBox Loss yields the best performance of 13:7 M, on par with RepGT with  = 1:0. Setting  as 0 means we completely smooth a ln function into a linear function and sum over IoU. We conjure that RepBox Loss tends to have more outliers than RepGT Loss since predicted boxes are much denser than ground-truth boxes. As mentioned in Section 1, detectors in crowd scenes are sensitive to the NMS threshold. A high NMS threshold may lead to more false positives, while a low NMS threshold may lead to more missed detections. In Figure 6 we show our results with RepBox Loss across various NMS thresholds at FPPI = . In general, the performance of detector with RepBox Loss is smoother than baseline. It is worth noting that at the NMS threshold of 0:35, the gap between baseline and RepBox is 3:5 points, indicating that the latter is less sensitive to NMS threshold. Through visualization in Figure 7, there are fewer predictions lying in between two adjacent ground-truths of RepBox. 


% \subsection{Occluded Pedestrian Detection}
% There are several ways to detect occluded pedestrians, \textit{e.g.,} end-to-end detection methods. The aforementioned methods directly map an image to a binary decision variable, resulting in a simplified procedure to detect occluded pedestrians. However, in this way, the deep learning model remains completely uninterpretable, which can be problematic for queries that rely on examining all sufficient reasons for making decisions.
% In this work, we model occluded pedestrian detection problems as a multi-class classification problem that yields better interpretability for final detection results than end-to-end detection methods.

% Let $\mathbf{x}$ be an input image, and $y$ be the corresponding label.
% Let $\mathbf{s}:=\{s_1, s_2, \cdots, s_n\}$ be the set of labels of body-parts used for training our deep neural model. When training is complete, given a test image, our model can predict the label of body-parts in terms of probability. We use $p(y=s \mid \mathbf{x})$ to denote the probability of a body part $s \in \mathbf{s}$ in a given image $\mathbf{x}$. Let $\Theta$ be a set of threshold values such that $\Theta:=\{\theta_s\}_{s=s_1}^{s_n}$. To detect a body-part in a test image $\mathbf{x}$, we define an indicator function $I_s$ as follows
% \begin{equation}\label{eqn:indicators}
%      I_s:= 
% \begin{cases}
%     1      & \text{if } p(y=s \mid \mathbf{x})\geq \theta_s,\\
%     0      & \text{otherwise},
% \end{cases}
% \end{equation}
% where $s\in \mathbf{s}$ represents a body-part.
% Note that we have not yet associated any decision variable which corresponds to the identification of pedestrian in an image frame. We do that now by using the indicator functions in Eqn. \eqref{eqn:indicators} as follows
% \begin{equation}\label{eqn:pedestrian}
%     \text{pedestrian} := 
%     \begin{cases}
%     1      & \text{if } \sum_s{I_s}>0,\\
%     0      & \text{otherwise}.
% \end{cases}
% \end{equation}
% As we can see from Eqn. \eqref{eqn:pedestrian}, our occluded pedestrian detection method works as an OR gate. We say an occluded pedestrian is detected if there exist a threshold value, $\theta_s \in \Theta$, for which the pedestrian variable in Eqn. \eqref{eqn:pedestrian} is $1$. 
% In summary, unlike end-to-end methods that do not provide semantic meaning for their results, our method disentangles underlying meaning of occlusion states by defining the detection probability over the body-parts. 


% % There are some methods for occluded pedestrian detection based on semantic feature extraction. These pedestrian detection are considered as binary classification.
% % In our proposed model we have used a multi class classification for part detection that enables a better interpret ability for final detection results.


% % of each parts and full body. We can set individual threshold value for each body parts and that help the model express results in a better way. Compare to binary classification our model has a multi class output followed by a OR function, and  the output of the OR function is a binary output. So, if our model can detect at least a single body parts, it can animate the results of existence of pedestrian. In case of partially visible pedestrian, our model can generate results with that OR function. If we consider P as our detection results, i is the class for body parts, and I is the threshold value, we can interpret our detection results as Equation 
% % \todo[inline]{Explain how do you detect pedestrians.}
% % outlines:



%     % \item the output of your model is a set of probabilities. you then need to define threshold values to determine body parts. Explain why a single threshold value is not a good idea to determine all body parts.
%     % \item Explain the trade-off between robustness and accuracy while selecting different values for thresholds.
%     % \item Explain your assumptions on occluded pedestrian detection and how your decision making algorithm works as ``OR'' function.
%     % \item Explain how your detection method entails safe navigation.

% % \begin{enumerate}
% % \end{enumerate}



==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/sect/conlude.tex <==
In this paper, we addressed the problem of occluded pedestrian detection in autonomous driving scenarios. A Single Shot Detection with Scale Specific Pooling Model (SSPM) is developed to accurately detect occluded pedestrians using their body parts. We also create a dataset for occluded pedestrian detection problem. With this dataset, we train a Feature Pyramid Network along with SSPM. The originality of the propose method is that it does not require a separate module to detect occluded pedestrian especially in autonomous driving scenarios. We are able to detect not only full body of the pedestrians, but also the different body parts in real time. Experimental results show that our proposed method outperforms the conventional SSD method. 
Further extension of this paper would be predicting the intention of pedestrians by detecting partial body parts. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textcolor{red}{As a future work we can consider developing a model based on parts detection. We can set some weight for different body parts and multiplying these weights with prediction score, we will have final score. Based on some predefined threshold value for final score of parts, we can develop a model to animate the full body if there is partial detection only.}

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/sect/exp.tex <==
\subsection{Dataset}
\todo[inline]{Please explain what is the problem of existing dataset and why do you need new dataset?}
% Selecting a proper dataset for training is a big challenge in object classification and localization \cite{soekhoe2016impact}. 
\textcolor{blue}{We have already mentioned that our pedestrian detection model is designed for improving detection accuracy for the occluded pedestrian. Though in most of the benchmark pedestrian dataset, there are some occluded pedestrians, those are not labeled for body parts separately. Some researchers also proposed CityPerson dataset as standard for occluded pedestrian \cite{zhang2018occluded}, but as those datasets are not labeled for body parts and labeling dataset is a tedious task, we took an initiative to create a small dataset of human body parts annotation within the full-body images. We have created a data set of human body parts for training our model that consists of 380 images, totaling around 1000 annotations for each different body parts and full body. We have taken 100 images from Penn-Fudan Database \cite{wang2007object}. For testing and evaluating our results, we have created a dataset of 613 images and 622 images of occluded pedestrians.} As some networks like Faster RCNN and SSD-mobilenet can provide satisfactory output with the small dataset we have performed our first training with a small data set. But, training with more body parts data will provide better detection results. We segregate the full body into three parts, namely head, hand, and leg.  We have collected half hand, full hand, a hand with a shoulder, thus covering the most body parts area. We tried to take our data with possible variations, such as taking data from different illuminations (Lights condition, indoor and outdoor as well), occlusion of parts data, and different sizes. Though our dataset is small, we tried to create variation by taking data from different places around the world including India, Bangladesh, Malaysia, Dubai, and the USA.
% We have add some additional raw images from Penn-Fudan Database \cite{wang2007object}, but we have used our own labeling.
\subsection{Training loss}
 %Training: 
\textcolor{blue}{Our training method is the same as the SSD training method, where we need to assign ground truth information to specific default outputs within the defined set of a default output. In the training procedure, our target is to determine the best-matched default boxes within a set of differently scaled bounding boxes for the given ground truth boxes. }
 \todo[inline]{say something related to supervised learning}
We have trained our model with a customized dataset of around 500 images those consists of more than 4000 annotations. We have run our training for around 42000 steps and stopped training after that. 
\todo[inline]{define and explain each loss in Fig. 5}
We showed the change of loss function with the number of steps in Fig. \ref{fig:Loss_function}. From Fig. \ref{fig:Loss_function}, we can see both classification loss and localization losses are gradually declining with the increase of no. of steps. \textcolor{blue}{The red and blue line shows localization loss and classification loss, respectively. The brown line shows the total loss, which is the sum of classification loss and localization loss.} 
\input{figtex/classification.tex}
\subsection{Case studies}
% As we have used the detector for pedestrians from the autonomous cars perspective we checked the result with a video file of pedestrian movement in front of a car. 
\todo{please explain how do you create the video file and what was your setup e.g., by using front-facing monocular camera...}

We have found that while we test the performance of SSD-Mobilenet, there is some false detection with pedestrian crossing signs where those are not actual pedestrians. Another issue is that, in the transition period of body movement, SSD-Mobilenet was unable to detect pedestrians for some of the frames (Figure \ref{fig:Compared result of two model_test_image_2}). On the other hand, While we have tested with our scale specific body parts detection model, for similar types of image frames, our detector can detect some body parts in the transition period and does not confuse by detecting a pedestrian in the pedestrian sign (Figure \ref{fig:Compared result of two model_test_image_2}). Hence, we can say that our model perform better in the case of transitional movement and false detection compared to SSD-mobilenet for particularly pedestrian detection. 
%Comparison results with the transition period are shown in Figure \ref{fig:Compared result of two %model_test_image_1}. 
% \input{figtex/comparison.tex}
% We have to compare different model with our data set and benchmark data set. 
% In analysis we have to describe the strong point of our newly developed model and specifically explained why this model is better than other model.
In our model for creating differently scaled feature maps, we used average pooling. We have tested with some sample images and found that average pooling consists of more information in the contrast region. During the day time, as most of the image has a high background intensity, average pooling performs better as compared to max-pooling. We have taken a sample pedestrian image with average intensity level and found that in the case of max pooling more information is lost as compared to average pooling (Fig. \ref{fig:Result comparison of max pooling_vs_avg_pooling_1}).

\input{figtex/max_pooling.tex}
Fig. \ref{fig:Result comparison of max pooling_vs_avg_pooling_2} shows that with a Max pooling operation, images having high intensity background lost more information compared to average pooling operation. Though max-pooling performed well in the case of a white object with a black background (Fig. \ref{fig:Result comparison of max pooling_vs_avg_pooling_3}), the average pooling result is also satisfactory. So, considering the different intensity levels in the images, average pooling provides more information as compared to max-pooling in the region of changing background intensity. 


\subsection{Performance analysis}
\todo[inline]{
you need to compute followings}
\begin{itemize}
    \item accuracy
    \item precision
    \item recall
    \item F-Score
    \item ROC curve
\end{itemize}
% As we did not find a benchmark dataset for result comparison, we have shown the accuracy of our model with a smaller dataset by checking the no. of objects detected correctly and no. of miss detections.
For analyzing the performance of our trained model we have selected a small dataset of 500 heads, 500 hands, and 470 legs parts and we have found around 93.19\% correct detections for leg, 88.2\% correct detection for hand and 90.8\% correct detection for the head. The correction percentages are pretty satisfactory. We have shown the result in Table \ref{table:Result comparison}. 

\input{figtex/table_result.tex}
We then compare our proposed model with SSD-Mobilenet for 613 image frames of fully visible pedestrians and considering at least one part or full body detection, our model outperforms SSD-Mobilenet model (Table \ref{table:Result comparison of visible dataset} ). 
\input{figtex/table_compare_normal_data_set}
Finally, we compare the performances between our proposed model and SSD-Mobilenet for a fully occluded dataset of 622 image frames and found our proposed model perform significantly better than SSD-Mobilenet for the occluded dataset (Table \ref{table:Result comparison of occluded dataset}).  
\input{figtex/table_dataset.tex}

\subsection{Runtime efficiency}
\todo[inline]{we need runtime comparison and we need to show that our proposed method is faster than SSD-Mobilenet.
}




==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/sect/intro.tex <==
Occluded pedestrian detection is a notoriously hard problem in autonomous driving scenarios. For the general pedestrian detection task, we have seen notable progress in computer vision algorithms throughout the last decade. In literature, we also have seen that deep neural networks based detection algorithms typically outperform classical rule-based detection algorithms \cite{zheng2012review, hou2018multispectral, zhao2016faster}. 
For instance, the state-of-the-art algorithm, 
% Deep Feature Pyramid Network (FPN),
SSD-mobilenet,
performs reasonably well in the real-world pedestrian detection problem and significantly better than rule-based approaches \cite{yao2018fully}.

Unfortunately, the occluded pedestrian problem is too challenging for SSD-mobilenet.
% and it appears that the much anticipated improvement in small scale object detection is still an open issue.
% the model used SSD, still has the scope of improvement with very small scale object detection. 
On the other hand, in the real world, occlusion happens very often. Therefore, it is crucial to detect occluded pedestrians using their body parts. Some efforts have been made to handle occlusion in autonomous driving either using a separate module to detect occluded pedestrians \cite{ouyang2013joint} or using a multishot image detector \cite{zhang2018occluded}. However, those methods are not desirable since our main goals for this paper are as follows:
1) to reduce the complexity of the detector and
2) to minimize supplementary computational resources. 

Consider the sudden pedestrian crossing scenario, which has always been a safety issue for autonomous driving. We argue that an autonomous vehicle can avoid such vehicle-pedestrian crashes if it could detect occluded pedestrians in real-time. To do that, given an image frame or a video stream, an occluded pedestrian detection method needs to identify which of a known set of body parts might be present and their corresponding positions within the image frame.

% \todo{explanation of SSD-Mobilenet}
Unlike other object detection methods, the Single Shot Detection (SSD) method takes only one single shot to detect multiple objects in the image frame. We are particularly interested here in the detection of occluded pedestrians with a single image shot. The key idea is to detect at least one body part of occluded pedestrian, which can then be localized in real-time speed.
% \todo{shortcoming of ssd-mobilenet}
In this paper, we have utilized the SSD-mobilenet as our base model. We then proposed a Scale Specific Pooling Model (SSPM), which is developed based on a set of average pooling layers and a set of predefined bounding boxes. We assume that pedestrians who appear too small in the image frame, are located far away from the vehicle. Detecting such pedestrians are not of our interest since they do not violate safety constraints for our application. Hence, we have proposed a set of predefined bounding boxes on top of a feature map to enhance the detection accuracy. Our proposed method is simple and easy to train. In our experiments, we show that our method can learn complex body parts as well as it can detect occluded pedestrians in real-time.


==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/sect/prelim.tex <==
% \todo{please write what do you explain in this section.}
In this paper, we have used the SSD-mobilenet as our base model. This model has two parts: Mobilenet \textendash used as the base network for classifying the object types, and SSD \textendash used for localizing the classified objects.

% \subsection{Mobilenet}
Having depth and pointwise separable output Mobilenet creates differs from the traditional convolutional neural networks which do not have separable outputs. 
% \input{figtex/cnn.tex}
Instead, Mobilenet is known as a depthwise separable convolutional network \cite{howard2017mobilenets}, which takes advantage of separable outputs from depthwise and pointwise convolution operations and reduces its complexity compared to other traditional convolutional neural networks. Figure~\ref{fig:Comparison of Convolution}(a) shows symbolic operation of traditional convolution versus depth and pointwise convolution operations  in Figures~\ref{fig:Comparison of Convolution}(b) and Figure~\ref{fig:Comparison of Convolution}(c) that are used in Mobilenet \cite{howard2017mobilenets}. 
\begin{figure}[h!]
    \centering
    \includegraphics[height=3.5cm, width = 8.5cm]{Figures/SSD-Feature_map.pdf}
    \caption{SSD Feature-map operation layers \cite{liu2016ssd}: (a) Input image with ground truth boxes, (b) 8x8 feature map showing default boxes with different aspect ratios those are generated by linearly mapped equation, and (c) 4x4 feature map showing default boxes with different aspect ratios.}
    \label{fig:SSD feature map}
  \end{figure}

% \subsection{Single Shot Detection (SSD)}
% Using the SSD after Mobilenet network, we add an auxiliary structure to the network to detect multi-scale feature maps and default boxes. 
Cascading the SSD with Mobilenet, we can detect multiple objects of different size.
SSD network provides bounding boxes and scores as output. Boxes indicate the location of the object and scores denote the probability of the detected object within the boxes. Training the SSD network with the multi-scale feature map provides the optimum bounding boxes for the detected objects \cite{liu2016ssd}. Figure \ref{fig:SSD feature map} shows the different feature map operation layers of SSD, in which Figure~\ref{fig:SSD feature map}(a) shows the ground truth boxes that are used for training, while Figure \ref{fig:SSD feature map}(b) and \ref{fig:SSD feature map}(c) show the set of default boxes with different feature maps. During the training of an SSD model,  the main goal is to match the default boxes with ground truth boxes \cite{liu2016ssd}. The matching of a default box is calculated using the overall loss function $L$, given in (\ref{loss}), in terms of the localization loss $L_{loc}$ and the confidence loss $L_{conf}$ \cite{liu2016ssd}:

\begin{equation}\label{loss}
    L(x,c,l,g)=(1/N)(L_{conf}(x,c)+\alpha L_{loc}(x,l,g)),
\end{equation}
 \noindent where $N$ is the number of matched default boxes and $\alpha$ is a weight term. The parameter $x$ contains the matching information  in the form of $x_{ij}^p =\{1,0\}$ which denotes whether the $i$\ts{th} default box from the the $p$\ts{th} category matches to the $j$\ts{th} ground truth box. The parameters  \textit{l} and \textit{g} contain the information about the predicted/ground-truth box boxes in the form of $l_{i}^m$ and $g_{i}^m$, where  $i$ refers to the $i$\ts{th} predicted/ground-truth box, and $m\in\{cx,cy, w,h\}$  refers to its parameters, where $c_x$ and $c_y$ are the coordinates of its center, $w$ is its width, and $h$ is its height. The parameter \textit{c} is the multiple class confidence, which contains the information in the form of $c_{i}^p$ which refers to the confidence level of belongings of $i$\ts{th} predicted box to the $p$\ts{th} category. Consider $d_{i}^m$, $m\in\{cx,cy, w,h\}$  a parameter of $i$\ts{th} default box and lets define $\hat{g}$ and $\hat{c}$  as follows:
 
  \begin{equation}\label{ghat}
\begin{split}
	\hat{g}_{j}^{cx} = (g_{j}^{cx} - d_{i}^{cx})/d_{i}^{w},   \hat{g}_{j}^{cy} = (g_{j}^{cy} - d_{i}^{cy})/d_{i}^{h} \\
	\hat{g}_{j}^{w} = log (g_{j}^{w}/d_{i}^{w}), 
	\hat{g}_{j}^{h} = log (g_{j}^{h}/d_{i}^{h})
	\end{split}
\end{equation}

   \begin{equation}\label{chat}
	\hat{c}_{i}^{p} = exp(c_{i}^p)/\sum_p exp(c_i^p)   
\end{equation}

\noindent Then, the localization loss $L_{loc}$ and confidence loss $	L_{conf}$ can be calculated as:

 \begin{equation}\label{loc_loss}
	L_{loc}(x,l,g)= \sum_{i \in Pos}^{N} \sum_{m} x_{ij}^k smooth_{L1} (l_{i}^{m} -\hat{g}_{j}^{m}) 
\end{equation}

\begin{equation}\label{conf_loss}
	L_{conf}(x,c)= - \sum_{i \in Pos}^{N} x_{ij}^{p} log(\hat{c}_{i}^{p}) - \sum_{i \in Neg} log(\hat{c}_{i}^{p})
\end{equation}
\noindent where $Pos$  is the set of indexes for default boxes which contain a detected object, referred to as positive default boxes, and $Neg$ is the set of indexes for default boxes which do not contain a detected object, referred to as negative default boxes.


Having the information about the bounding boxes and scores as outputs of SSD, a non-maximum suppression \cite{rothe2014non} step is used as a post-processing step to produce the final detection, which helps to identify the highest probable object within a single bounding box. 

\begin{figure}[htb]
    \centering
  
    \includegraphics[width=8cm]{Figures/ssd-architecture.pdf}
    

  \caption{Architecture of the SSD-Mobilenet Model \cite{jin2018pooling}.}
  \label{fig:Structure of SSD-Mobilenet Model}
\end{figure}
% Review of part based model if any, address the problem of those methods

% How I am addressing those problem identified in earlier section. 
Figure \ref{fig:Structure of SSD-Mobilenet Model} shows the overall architecture of SSD-Mobilenet. It starts with a MobileNet processing, followed by multi-scale feature maps, which generate bounding boxes and scores as outputs of the network. 
On the development of SSD, Pooling Pyramid Network first introduces the shared tower concept for predicting box score and box location instead of individual box score and box location from differently scaled feature map layers \cite{jin2018pooling}.



%This model has been trained to detect around 90 different types of objects and this model works satisfactorily while it is used for pedestrian detection only. But we found some miss detection in the transition time of pose change. If we trained our proposed model for different body parts, the detector can detect few body parts during the transition time of pose change or movement that enables us to distinguish the performance of the proposed model with the body part detection to full-body detection with SSD-Mobilenet.  
%

==> SMC2021-EXtended8p-Pedestrian Detection by Fusing Camera and LiDAR-V1/sect/related.tex <==
% Different Method, Classical, CNN, Pros and cones, why learning is good method: 
Vision-based pedestrian detection can be categorized into two groups:  static pedestrian detection  and dynamic pedestrian detection \cite{zheng2012review}. In this work, we focus on dynamic pedestrian detection, especially occluded pedestrian, using a supervised learning technique.
% \todo[inline]{What kind of pedestrian detection do you propose ... }
\subsection{Classical Methods}
% \textemdash which is a combination of multiple features, and part-based pedestrian detection
% \textemdash which is divided into two groups of model-based and feature-classifier-based),

% \todo[inline]{please Write some glue texts related to classical methods.} Classical method of pedestrian detection or feature based pedestrian detection create a milestone in the development pedestrian detection. One of the major parts of pedestrian detection is feature extraction. 
Classical method can be divided into two groups \textemdash model-based and features-classifier-based pedestrian detection. \todo[inline]{Explain model based detection} .Typically, classical methods employ handcrafted feature extraction to determine pedestrians. Some powerful feature extractors used for pedestrian detection using classical approached are Histogram of Oriented Gradient (HOG)\cite{dalal2005histograms}, Histogram of Oriented Flow (HOF)\cite{dalal2006human}, Scale Invariant Feature Transform (SIFT)\cite{wang2010boosting}, Covariance \cite{paisitkriangkrai2008fast}\cite{tuzel2006region}\cite{gualdi2009covariance}, Haar Wavelet\cite{oren1997pedestrian}, Hierarchical Max (HMAX)\cite{gu2009modified}, and Local Binary Patterns (LBP)\cite{mu2008discriminative}.
% \todo[inline]{Please focus on pedestrian detection problem only, not feature extractions ... }
Although static shape features based pedestrian detection provides a very good platform for pedestrian detection, lacks performance in the scenario of  dynamic shape and varying poses of the pedestrians. Feature-classifier-based detector outperforms the shape model-based pedestrian detectors, but except for the HMAX feature classifiers, all of the other feature classifiers are highly dependent on the large number of training data\cite{zheng2012review}. In \cite{baek2019pedestrian}, combining with binarized normed gradient (BING) method \cite{cheng2014bing}, authors propose the additive kernel support vector
machine (AKSVM) that provides competitive detection speed by generating efficient region proposal. Some researchers combine different features to improve the performance as compared to that of the single feature-based classifiers.
\textcolor{red}{
%In \cite{szarvas2005pedestrian}, a Convolutional Neural Network has been used to detect pedestrians which outperforms detectors with classical feature extractors and classifiers \cite{dalal2005histograms}.
However, classical feature extractors and classifiers for pedestrians detection are not performing satisfactorily in the case of dynamic scenario, occluded pedestrian, and with a different appearance of pedestrians. Hence, we considered a deep learning network to detect occluded pedestrian for the autonomous car.
} 

\todo[inline]{Limitation of handcrafted feature. Please explain the limitation of classical methods and why don't you adopt one of them (from autonomous vehicle point of view)}.

\subsection{Deep Neural Network Based Methods}

% \todo[inline]{please Write some glue texts related to Deep learning.}
Deep learning based pedestrian detection methods have created a milestone by improving performance in pedestrian detection with varies illumination level and complex background with multiple pedestrians. In literature, we have seen convolution neural networks, \textit{e.g.,} R-CNN, Fast-RCNN, Faster R-CNN and SSD-Mobilenet are utilized for pedestrians detection.
To localize an pedestrian in an image, R-CNN \cite{zhang2018occlusion} model combines the \emph{region proposal} method  with CNNs. That region proposal method uses a search algorithm to find candidate regions and then, each region is fed into the CNN network. However, R-CNN model is very slow due to the high computation cost of the search algorithm. To reduce the computation cost, instead of feeding the each region into CNN network separately, Fast-RCNN \cite{girshick2015fast} model feeds the full image  along with the proposed regions resulted from the search algorithm into the CNN network. Faster-RCNN \cite{ren2015faster} implements an improved version of Fast-RCNN by eliminating the search algorithm with a separate network for region proposal. Instead of searching over different regions of an image frame over two steps/networks, Yolo \cite{redmon2016you} uses a single network object detection with the bounding box. 
\subsubsection{Pyramid Network}
Another single network detector has been introduced in \cite{liu2016ssd}, known as Single Shot Multibox Detector (SSD). In SSD, feature maps with different scales, help it to detect different sized objects in a convolutional fashion. Some development on SSD is the Feature Pyramid Network (FPN) \cite{lin2017feature} and Pooling Pyramid Network (PPN) \cite{jin2018pooling}.
% Different Methods for occlusion handling problem, problem of those methods. Why part based occlusion handling method is better. 
Though the different CNN model has created a milestone in object detection, especially in pedestrian detection, a problem like occlusion handling is still a concerning issue which has significant importance for autonomous car and other surveillance systems. Joint Deep Learning model\cite{ouyang2013joint} provides a solution for occlusion handling, but this model is sensitive to localize the pedestrian and slow as, well as this model is not depth-wise separable. Another problem with the deep part model is that this model tried to find out the occluded body parts based on some predefined body structure which is sensitive to pose variation.

\subsubsection{Mobilenet}
SSD-Mobilenet in \cite{howard2017mobilenets} has been prepared for detecting multiple (around 90 different) types of objects. The main challenge with SSD-Mobilenet is that if it is trained for a particular object like a pedestrian, it can not detect pedestrians with some variation of poses, some of the deformed shapes of pedestrians, and partially occluded pedestrians. Besides, if we use SSD-Mobilenet for pedestrian detection, it detects similar types of pedestrian shapes as pedestrian, e.g., it may detects a symbol of pedestrian crossing sign as a pedestrian which creates confusion between real pedestrians and objects similar to a pedestrian. For the steady operation of the autonomous car, it is important to detect the visible parts of the pedestrian if pedestrians' full bodies are not visible. So, we proposed a method for pedestrian detection that can detect pedestrians, along with pedestrians' body parts using the same network.

% \todo[inline]{inspiration of the proposed method and how it works}

Inspired by SSD-Mobilenet and Pooling Pyramid Network (PPN), we proposed a Scale Specific Pooling (SSP) model, which combines a separable network and a shared prediction layer for pedestrian detection.
% \todo{What do you combine?}
One of the major changes in our proposed model compared to SSD-Mobilenet is the replacement of convolution between feature maps with average pooling layers and we have done this differently scaled average pooling based on expected object sizes and ground truth box sizes.


% Organization of the paper. 
% The following section describes the background of the machine vision application for pedestrian detection, then the proposed scale specific model that we have created by tuning some hyperparameters and changing layer sizes for more specific detection is explained. After that, in the discussion section, we show the result that provides better decision-making ability for autonomous cars by detecting body parts of pedestrians in front of the car. Finally, some of the possible areas to improve detector performance have been discussed. 


==> config/packages_old.tex <==

%% Added Package
% amsmath and amssymb packages, useful for mathematical formulas and symbols
\usepackage{amsmath,amssymb,graphicx,breqn}
% for adding definition in writing
\usepackage{amsfonts,amsthm,epsfig,epstopdf,titling,url,array}

% cite package, to clean up citations in the main text. Do not remove.
\usepackage[noadjust]{cite} % for [] - [] citation
% \usepackage[sort&compress]{cite}
\bibliographystyle{ieeetr} % From outside Calling
% Use nameref to cite supporting information files (see Supporting Information section for more info)
\usepackage{url,nameref}
%\usepackage[hidelinks=true]{hyperref} % For Referencing without box
\usepackage{hyperref} % For Referencing but red box
% \usepackage[hidelinks=true]{hyperref} % For Referencing

\usepackage{setspace} % for controlling spacing in line
\usepackage{color}
\usepackage{ragged2e} % For Justification

% color can be used to apply background shading to table cells only
\usepackage[table]{xcolor}

% for adding definition in writing
\theoremstyle{plain}
\newtheorem{thm}{Theorem}%[section]
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem*{cor}{Corollary}

\theoremstyle{definition}
\newtheorem{defn}{Definition}%[section]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{exmp}{Example}%[section]

\newtheorem{rem}{Remark}%[section]

\theoremstyle{remark}
%\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}


% Figure Purpose
\usepackage{graphicx}
\usepackage{subcaption}

% For Caption Legend adding purpose
\usepackage{color}
\usepackage{tikz}
\usetikzlibrary{shapes}

%In case you encounter the following error:
%Error 1010 The PDF file may be corrupt (unable to open PDF file) OR
%Error 1000 An error occurred while parsing a contents stream. Unable to analyze the PDF file.
%This is a known problem with pdfLaTeX conversion filter. The file cannot be opened with acrobat reader
%Please use one of the alternatives below to circumvent this error by uncommenting one or the other
%\pdfobjcompresslevel=0
%\pdfminorversion=4

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document

% The following packages can be found on http:\\www.ctan.org
%\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%\usepackage{amsmath} % assumes amsmath package installed
%\usepackage{amssymb}  % assumes amsmath package installed



==> figtex/architecture.tex <==
%% Creator: Inkscape inkscape 0.92.4, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'architectureGradient.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To Scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{309.64281878bp}%
    \ifx\svgScale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgScale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgScale\undefined%
  \makeatother%
  \begin{picture}(1,1.10224947)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength]{figtex/architecture.eps}}%
   \put(0.163438817,0.2005536){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Conv\end{tabular}}}}%
    \put(0.0922034,0.44100306){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Average Pooling\end{tabular}}}}%
    \put(0.0922034,0.68204425){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Average Pooling\end{tabular}}}}%
    \put(0.0922034,0.92760688){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Average Pooling\end{tabular}}}}%
    
    %%%standard
    \put(0.07922034,0.31941654){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1\ts{st} Scale Feature Map\end{tabular}}}}%
    \put(0.07922034,0.56290941){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}2\ts{nd} Scale Feature Map\end{tabular}}}}%
    \put(0.07922034,0.80290707){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}3\ts{rd} Scale Feature Map\end{tabular}}}}%
    \put(0.07922034,1.04812196){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}4\ts{th} Scale Feature Map\end{tabular}}}}%
    
    
    \put(0.595422909,0.67666367){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Shared\\ Tower\end{tabular}}}}%
    \put(0.863341397,0.79304843){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}  Box\\Score\end{tabular}}}}%
    \put(0.863341397,0.54578977){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}   Box\\Location\end{tabular}}}}%
    \put(0.122034,0.08006312){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Base Network\\(MobileNet)\end{tabular}}}}%
  
  \end{picture}%
\endgroup%


==> figtex/classification.tex <==

% \begin{figure}[h!]
%     % \includegraphics[trim={0,0,0,2cm},clip,width=8.65cm]{mashuk/Images/Loss_function.png}
%     \includegraphics{mashuk/Images/Loss_function.png}
%     \caption{Losses during training, run across $42k$ epochs. The red, green and blue lines represent total loss, localization loss and classification loss, respectively. }
%     \label{fig:Loss_function}
%   \end{figure}
 
 
 \begin{figure}[h!]

\begin{tikzpicture}
\begin{axis}[
xlabel={Number of epochs},
ylabel = {Loss}
]
  
\addplot table [x=No. of steps, y=Classification loss, col sep=comma] {resources/graph.csv};

\addplot table [x=No. of steps, y=Localization loss, col sep=comma] {resources/graph.csv};

\addplot table [x=No. of steps, y=Total loss, col sep=comma] {resources/graph.csv};

\legend{Classification loss,Localization loss,Total loss};

\end{axis}
\end{tikzpicture}
    \caption{Losses during training, run across $42\times 10^3$ epochs. The red, green and blue lines represent total loss, localization loss and classification loss, respectively. }
    \label{fig:Loss_function}
  \end{figure}

==> figtex/cnn.tex <==
\begin{figure}[h!]
    \centering
    \vspace{4mm}
  \includegraphics[width=8.65cm]{Images/Mobilentet_conv.jpg}
  \caption{Comparison of Mobilenet convolutional operation with traditional Convolutional Operation \cite{howard2017mobilenets}: (a) Traditional convolution, (b) depthwise convolution, and (c) point-wise convolution operations in the context of Depthwise Separable Convolution.}
  \label{fig:Comparison of Convolution}
\end{figure}


==> figtex/miss_rate_fppi_curve.tex <==
\begin{figure}[htb]
    \centering
    \vspace{-5pt}
    \includegraphics[width= 9cm]{Figures/benchmark.png}
    \caption{\small{The comparison among Fused-YOLO, Fusion without applying Kalman Filter, and Baseline YOLOv5. Fused-YOLO model get the lowest miss rate of $33.435\%$ among others.}\small{The comparison among Fused-YOLO, Fusion without applying Kalman Filter, and Baseline YOLOv5. Fused-YOLO model get the lowest miss rate of $33.435\%$ among others.}}
    \label{fig:Miss_rate_vs_fppi}
    \vspace{-5pt}
\end{figure}

==> figtex/miss_rate_fppi_curve2.tex <==
% \begin{figure}[htb]
%     \centering
%     \vspace{-5pt}
%     \includegraphics[width= 9cm]{Figures/benchmark.png}
%     \caption{\small{The comparison of Fused-YOLO with YOLOv5. Fused-YOLO model get a lower miss rate compare to YOLOv5 model.}}
%     \label{fig:Miss_rate_vs_fppi}
%     \vspace{-5pt}
% \end{figure}

\begin{figure}[htb]
\begin{tikzpicture}
\begin{axis}[
    axis lines=middle,
    axis line style={->},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    xlabel={FPPI},
    ylabel={Miss Rate},
    xmin=0, xmax=1,
    ymin=0, ymax=0.6,
    xtick={0.2, 0.4, 0.6, 0.8, 1.0},
    xticklabels={$10^{-3}$,$10^{-2}$, $10^{-1}$, $10^{0}$, $10^{1}$ },
    ytick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
    legend pos=north east,
    ]
\addplot [color=blue, line width=1.6pt] table [x=x, y=y, col sep=comma] {resources/Fused-Yolo.csv};
\addlegendentry{Fused-Yolo (33.435)\%}
\addplot [color=darkgray,dashed, line width=1.6pt] table [x=x, y=y, col sep=comma] {resources/Fusion without KF.csv};
\addlegendentry{Fusion without KF (38.602)\%}
\addplot[color=red,dashed, line width=1.6pt] table [x=x, y=y, col sep=comma] {resources/Baseline method.csv};
\addlegendentry{Baseline method (41.945)\%}
\end{axis}
\end{tikzpicture}
    \caption{\small{The comparison among Fused-YOLO, Fusion without applying Kalman Filter, and Baseline YOLOv5. Fused-YOLO model get the lowest miss rate of $33.435\%$ among others.}}
    \label{fig:Miss_rate_vs_fppi}
\end{figure}

==> figtex/mobilnet.tex <==


% \begin{figure}[htb]
%   \includegraphics[width=8.65cm]{Images/SSD-Mobilenet.png}

%   \caption{Architecture of the SSD-Mobilenet Model \cite{jin2018pooling}.}
%   \label{fig:Structure of SSD-Mobilenet Model}
% \end{figure}

==> figtex/ssd-mobilenet.tex <==
%% Creator: Inkscape inkscape 0.92.4, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'ssd-mobilenet.eps' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{280.54945319bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.29970606)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength]{figtex/ssd-mobilenet.eps}}%
    
    % scale feature map
    \put(0.05128073,0.1845645){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1\ts{st} Scale Feature Map\end{tabular}}}}%
    \put(0.05128073,0.46453721){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}m\ts{th} Scale Feature Map\end{tabular}}}}%
    \put(0.03,0.734292){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(m+1)\ts{th} Scale Feature Map\end{tabular}}}}%
    \put(0.05128073,1.16140364){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}N\ts{th} Scale Feature Map\end{tabular}}}}%
    
    % conv
    \put(0.179113,0.6091571){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Conv\end{tabular}}}}%
    \put(0.179113,1.0317062){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Conv\end{tabular}}}}%
    
    % tower
    \put(0.603256874,0.22543618){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1\ts{st}\\tower\end{tabular}}}}%
    \put(0.603256874,0.7915123){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}m\ts{th}\\tower\end{tabular}}}}%
    \put(0.603256874,0.51153959){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(m+1)\ts{th}\\tower\end{tabular}}}}%
    \put(0.603256874,1.19818794){\color[rgb]{1,1,1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}N\ts{th}\\tower\end{tabular}}}}%
    
    % box location
    \put(0.85841522,0.12573624){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    \put(0.85841522,0.40775252){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    \put(0.85841522,0.70694323){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    \put(0.85841522,1.10340087){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Location\end{tabular}}}}%
    
    % box score
    \put(0.85841522,0.27900572){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    \put(0.85841522,0.56306556){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    \put(0.85841522,0.85325627){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    \put(0.85841522,1.24971395){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Box\\Score\end{tabular}}}}%
    
    % base net
    \put(0.1457859,0.10581671){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Base Network\\(MobileNet)\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> figtex/ssd.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics{Images/SSD_feature_map.jpg}
    \caption{SSD Feature-map operation layers \cite{liu2016ssd}: (a) Input image with ground truth boxes, (b) 8x8 feature map showing default boxes with different aspect ratios, and (c) 8x8 feature map showing default boxes with different aspect ratios.}
    \label{fig:SSD feature map}
  \end{figure}

==> figtex/table_compare_normal_data_set.tex <==
  \begin{table}[h!]
   \caption{Result comparison between SSD-Mobilenet and proposed method for fully visible pedestrians}
    \label{table:Result comparison of visible dataset}
    \begin{center}
    \begin{tabular}{|c||c||c||c|}
    \hline
    Model name & Correct detection & Miss detection & Perc. correct\\
    \hline
    SSD-Mobilenet & 526 & 87 & 85.80 \\ % inserting body of the table
    \hline
    Proposed method & 594 & 19 & 96.9 \\
    \hline
    \end{tabular}
    \end{center}
\end{table}

==> figtex/table_dataset.tex <==
\begin{table}[h!]
    \caption{Result comparison between SSD-Mobilenet and proposed method for occluded dataset}
    \label{table:Result comparison of occluded dataset}
    \begin{center}
    \begin{tabular}{|c||c||c||c|}
    \hline
    Model name & Correct detection & Miss detection & Perc. correct\\
    \hline
    SSD-Mobilenet & 292 & 330 & 46.94 \\ % inserting body of the table
    \hline
    Proposed method & 594 & 28 & 95.49 \\
    \hline
    \end{tabular}
    \end{center}
\end{table}

==> figtex/table_result.tex <==
\begin{table}[h]
    \caption{Result analysis with some fixed frames}
    \label{table:Result comparison}
    \begin{center}
    \begin{tabular}{|c||c||c||c|}
    \hline
    Object types & No. of Objects & Correct & Incorrect\\
    \hline
    Head & 500 & 454 & 46 \\ % inserting body of the table
    \hline
    Hand & 500 & 441 & 59 \\
    \hline
    Leg & 470 & 438 & 32 \\ 
    \hline
    \end{tabular}
    \end{center}
    \end{table}
    

==> sect/algo.tex <==

% %While testing our autonomous car, we figured out that some existing models of pedestrian detectors such as SSD-Mobilenet and Faster R-CNN confuse actual pedestrian with pedestrian crossing signs. Those models are trained with robust data sets and detect the pedestrian symbol within the pedestrian crossing sign, due to which detector can not distinguish between actual pedestrian and pedestrian crossing signs, which creates problems in decision making for the autonomous car. To overcome this problem, we have created a scale specific model to detect only the objects with expected size and those are actual pedestrians. In machine vision, object detection is challenging in many aspects, such as training data set creates a huge impact on detection specification. The preferred size of the desired object can be tuned by the model architecture. Based on the idea of specific or some desired expected output object size, we have tuned one of the well-known models. SSD-Mobilenet-V1 has been used for up to 90 different types of objects. But, we have trained that modified model for pedestrian detection only.  As the depth of the model is reduced, it speeds up the trained model detection performances. %
% So far we have explained the architecture of our base network.
% In this section, we explain our proposed method for pedestrian detection based on partial body parts. 

% % This allows within deformed shapes and occluded conditions. \todo{Not a complete sentence, please rewrite it.}
% % The proposed method also does not get confused by detecting pedestrian-like objects (those that are not actual pedestrians) by classifying them as a pedestrian. \todo{How do you validate this?}

% \subsection{Scale Specific Pooling operation (SSPO)}
% \input{figtex/sspm.tex}
% % Inspired by SSD-Mobilenet and Pooling Pyramid Network (PPN),  this section describes our proposed Scale Specific Pooling (SSP) model.  One of the major changes in our proposed model compared to SSD-Mobilenet is the replacement of convolution between feature maps with average pooling layers and we have done this differently scaled average pooling based on expected object sizes and ground truth box sizes.
% %\textcolor{red}{Inspired by PPN, We have used a shared tower for predicting box scores and locations for different body parts types.} This section also describes the effect of feature extraction for different body parts of the pedestrian compares to full body pedestrians. \textcolor{red}{We have made our model less complex and specific object detection oriented.}

% Scale Specific Pooling operation starts after the Mobilenet base network. 
% When we cascade Mobilenet with proposed SSPM the main adventage is, the combination reduces the scale factors in the images. In SSPM, we add convolutional feature layers and pooling layers to the end of our base network. These layers in FPN reduce the size progressively at different scales. We use some specific scale sizes average pooling for extracting different scale feature maps based on our training data and expected object sizes in test images. The differently scaled average pooling feature maps that we have used in our model are sized of $2\times2$, $4 \times 4$, $8 \times 8$ and $16 \times 16$. We trained our network with the pedestrian full body along with three body parts, and these consist of four different label IDs for each category. Training with body parts helps the model to extract more precise information about pedestrians.
% % \todo[inline]{explain how to train}
% %In our test, we assume the expected distance of pedestrians from the car is around 10m to 50m. Hence, 

% In SSPM, each feature layers can absolutely produce a fixed set of prediction maps with the help of convolutional filter and average pooling operation. The output of SSPO is a set of bounding boxes which got deafult sizes with each cell from each feature map. 
% Figure \ref{fig:Scale Specific Pooling Model} shows the structure of our proposed model.
% % After extracting feature information from the image using the mobilenet, our model takes a convolutional operation for generating the $1^{st}$  scale feature map. Then having three successive average pooling operations, we will have $2^{nd}$, $3^{rd}$ and, $4^{th}$ feature map layers. These feature maps use a shared tower to generate their prediction information. In our case, these shared towers consist of the information of the full body and three different body parts captured in different feature maps. 

 
% %From the mobilenet We have replaced the convolution operation with average pooling for different feature map layers, we have avoided addition and multiplication operation involving in convolution operation. Hence, the complexity of our model is reduced. We have used some specific scale sizes average pooling for extracting different scale feature maps as our model is trained for detecting only three different body parts (head, hand, and leg) along with full body of pedestrian, whereas SSD-Mobilenet is trained for ninety different types of object detection \textcolor{red}{with lot of variation in sizes.} As in this paper we consider pedestrian detection from a autonomous car's perspective, we want to detect the pedestrian while they are not a long distance from the car and considered the object size should not that small. The expected distance of pedestrian from the car that we considered in our test is around 10m to 50m. Considering the size of expected pedestrian body parts, the four pooling feature maps that we have used in our model are sized of 2 $\times$ 2, 4 $\times$ 4, 8 $\times$ 8 and 16 $\times$ 16. While we have trained our model, we have to make sure that the ratio of our highest scaled average pooling sizes, should grater than the ratio of the input image to the minimum sized ground truth box. So, the minimum sized ground truth box should be smaller in size compared with the smallest default box. On the other hand, to avoid false detection with a very small-sized object, we have considered our highest pooled feature map as 16 $\times$ 16.

% \subsection{Shared Tower}
% %\textcolor{red}{We can see from the architecture of SSD-Mobilenet shown in Figure \ref{fig:Structure of SSD-Mobilenet Model}, that the box scores and box locations are calculated for different feature layers, whereas }
% Shared towers consist of the information of the full body and three different body parts captured in different feature maps. 
% It is connected with each feature map layers and consists of feature information of the same location with different feature maps.
% % (Figure \ref{fig:Scale Specific Pooling Model}), which is similar to PPN model.
% Then it combines differently scaled feature maps to predict the final box score and its corresponding location. Thus, the shared tower provides classified object's score and bounding box location comparing the classified object's scores and bounding boxes of different feature map's output.
% % \todo[inline]{please provide more information}
% % As we have used shared box predictor in our model, that avoid miscalibration of score prediction with different scale as in case of with SSD-Mobilent \cite{jin2018pooling}. 


% %To overcome the problem with occlusion handling and pose variation, in our pedestrian detection model we have considered using three different body parts along with full body and the model consists of four different label IDs for three different body parts and a full body. So, feature extraction is more precise in the case of body parts compared to full body feature extraction. \textcolor{red}{While we trained our model with pedestrian body parts, the model consists of more precise information of the three body parts compared to a pedestrian detection model with a single ID.} For example, in the case of full-body pedestrian detection with SSD-Mobilenet, we found the model sometimes failed to detect the pedestrian while there is not enough gap between legs and hands are not stretch enough from the body. On the other hand in a similar scenario, the model with part detection can at least detect some body parts, though it can not detect the full body \ref{fig:Compared result of two model_test_image_2}. Our proposed model can detect the body parts as the model has more feature information for body parts. We have also set different threshold value for different body parts and these threshold value act like an weights for final detection, 
% %%
% %\subsection{Scale Specific pooling Model Architecture}
% %The architecture of the scale-specific model is very similar to the Pooling Pyramid Network(PPN), which is another modification of SSD-Mobilenet-V1. However, in pedestrian detection, we expect the size of our objects should not that small which is considered in SSD-Mobilenet for 90 different types of object detection. Hence, instead of taking various scaling as used in the SSD-mobilenet, in our model, for creating different feature maps, we have taken three specific ratios. On the other hand, we take all of our bounding boxes in the training dataset to be more than 28x56 pixel size and hence we consider average pooling for the different scaling features.

% %\begin{figure}[h!]
%  % \includegraphics{Images/Images1.jpg}
%  % \caption{Structure of SSD-Mobilenet Model\cite{jin2018pooling}}
%  % \label{fig:Structure of SSD-Mobilenet Model}
% %\end{figure}
% %We can see from the architecture of SSD-Mobilenet-V1 Figure \ref{fig:Structure of SSD-Mobilenet Model}, that the box scores and box locations are calculated for different feature layers whereas in scale specific pooling model we have used the shared tower for differently scaled feature maps to get the finalized box score and box location as in the case of PPN \cite{jin2018pooling}. Using SSD-Mobilenet, for pedestrian detection, we have found that there is some false detection with small scale object detection. To avoid the confusion with these small size object detection, we have designed our model to work with some specific scale only. We got better results with the scale size of 10x10, 5x5, 3x3 and 1x1 shown in Figure \ref{fig:Scale Specific Pooling Model}. 
% %\begin{figure}[h!]
%  % \includegraphics[width=8.65cm]{Images/scale_s_pooling.jpg}
%  % \caption{Structure of Scale Specific Pooling Model}
%  % \label{fig:Scale Specific Pooling Model}
% %\end{figure}
% %Instead of using a full-body dataset, we have used the body parts dataset for pedestrian detection. In the case of an occluded pedestrian, the detector used for full-body detection is not able to detect the object often, whereas our model which is trained with body parts, can detect some visible parts of the body to provide an idea about the actual object. As we eliminate the low scaling feature map layer and use average pooling instead of max pooling, it provides us more accurate information in the output layer. Average pooling captures more information as compared to max pooling, while there is a drastic change in intensity levels within the image.  

% % \subsection{Addition of repulsion loss}
% % We add repulsion loss for different body parts and detect the body parts more accurately in a crowded scenario. RepBox Loss. For RepBox Loss, we experiment with a different smooth parameter , reported in the fourth line of Table 1. When setting  as 0, RepBox Loss yields the best performance of 13:7 M, on par with RepGT with  = 1:0. Setting  as 0 means we completely smooth a ln function into a linear function and sum over IoU. We conjure that RepBox Loss tends to have more outliers than RepGT Loss since predicted boxes are much denser than ground-truth boxes. As mentioned in Section 1, detectors in crowd scenes are sensitive to the NMS threshold. A high NMS threshold may lead to more false positives, while a low NMS threshold may lead to more missed detections. In Figure 6 we show our results with RepBox Loss across various NMS thresholds at FPPI = . In general, the performance of detector with RepBox Loss is smoother than baseline. It is worth noting that at the NMS threshold of 0:35, the gap between baseline and RepBox is 3:5 points, indicating that the latter is less sensitive to NMS threshold. Through visualization in Figure 7, there are fewer predictions lying in between two adjacent ground-truths of RepBox. 


% \subsection{Occluded Pedestrian Detection}
% There are several ways to detect occluded pedestrians, \textit{e.g.,} end-to-end detection methods. The aforementioned methods directly map an image to a binary decision variable, resulting in a simplified procedure to detect occluded pedestrians. However, in this way, the deep learning model remains completely uninterpretable, which can be problematic for queries that rely on examining all sufficient reasons for making decisions.
% In this work, we model occluded pedestrian detection problems as a multi-class classification problem that yields better interpretability for final detection results than end-to-end detection methods.

% Let $\mathbf{x}$ be an input image, and $y$ be the corresponding label.
% Let $\mathbf{s}:=\{s_1, s_2, \cdots, s_n\}$ be the set of labels of body-parts used for training our deep neural model. When training is complete, given a test image, our model can predict the label of body-parts in terms of probability. We use $p(y=s \mid \mathbf{x})$ to denote the probability of a body part $s \in \mathbf{s}$ in a given image $\mathbf{x}$. Let $\Theta$ be a set of threshold values such that $\Theta:=\{\theta_s\}_{s=s_1}^{s_n}$. To detect a body-part in a test image $\mathbf{x}$, we define an indicator function $I_s$ as follows
% \begin{equation}\label{eqn:indicators}
%      I_s:= 
% \begin{cases}
%     1      & \text{if } p(y=s \mid \mathbf{x})\geq \theta_s,\\
%     0      & \text{otherwise},
% \end{cases}
% \end{equation}
% where $s\in \mathbf{s}$ represents a body-part.
% Note that we have not yet associated any decision variable which corresponds to the identification of pedestrian in an image frame. We do that now by using the indicator functions in Eqn. \eqref{eqn:indicators} as follows
% \begin{equation}\label{eqn:pedestrian}
%     \text{pedestrian} := 
%     \begin{cases}
%     1      & \text{if } \sum_s{I_s}>0,\\
%     0      & \text{otherwise}.
% \end{cases}
% \end{equation}
% As we can see from Eqn. \eqref{eqn:pedestrian}, our occluded pedestrian detection method works as an OR gate. We say an occluded pedestrian is detected if there exist a threshold value, $\theta_s \in \Theta$, for which the pedestrian variable in Eqn. \eqref{eqn:pedestrian} is $1$. 
% In summary, unlike end-to-end methods that do not provide semantic meaning for their results, our method disentangles underlying meaning of occlusion states by defining the detection probability over the body-parts. 


% % There are some methods for occluded pedestrian detection based on semantic feature extraction. These pedestrian detection are considered as binary classification.
% % In our proposed model we have used a multi class classification for part detection that enables a better interpret ability for final detection results.


% % of each parts and full body. We can set individual threshold value for each body parts and that help the model express results in a better way. Compare to binary classification our model has a multi class output followed by a OR function, and  the output of the OR function is a binary output. So, if our model can detect at least a single body parts, it can animate the results of existence of pedestrian. In case of partially visible pedestrian, our model can generate results with that OR function. If we consider P as our detection results, i is the class for body parts, and I is the threshold value, we can interpret our detection results as Equation 
% % \todo[inline]{Explain how do you detect pedestrians.}
% % outlines:



%     % \item the output of your model is a set of probabilities. you then need to define threshold values to determine body parts. Explain why a single threshold value is not a good idea to determine all body parts.
%     % \item Explain the trade-off between robustness and accuracy while selecting different values for thresholds.
%     % \item Explain your assumptions on occluded pedestrian detection and how your decision making algorithm works as ``OR'' function.
%     % \item Explain how your detection method entails safe navigation.

% % \begin{enumerate}
% % \end{enumerate}



==> sect/conlude.tex <==
In this paper, we addressed the problem of occluded pedestrian detection in autonomous driving scenarios. A Single Shot Detection with Scale Specific Pooling Model (SSPM) is developed to accurately detect occluded pedestrians using their body parts. We also create a dataset for occluded pedestrian detection problem. With this dataset, we train a Feature Pyramid Network along with SSPM. The originality of the propose method is that it does not require a separate module to detect occluded pedestrian especially in autonomous driving scenarios. We are able to detect not only full body of the pedestrians, but also the different body parts in real time. Experimental results show that our proposed method outperforms the conventional SSD method. 
Further extension of this paper would be predicting the intention of pedestrians by detecting partial body parts. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textcolor{red}{As a future work we can consider developing a model based on parts detection. We can set some weight for different body parts and multiplying these weights with prediction score, we will have final score. Based on some predefined threshold value for final score of parts, we can develop a model to animate the full body if there is partial detection only.}

==> sect/exp.tex <==
\subsection{Dataset}
\todo[inline]{Please explain what is the problem of existing dataset and why do you need new dataset?}
% Selecting a proper dataset for training is a big challenge in object classification and localization \cite{soekhoe2016impact}. 
\textcolor{blue}{We have already mentioned that our pedestrian detection model is designed for improving detection accuracy for the occluded pedestrian. Though in most of the benchmark pedestrian dataset, there are some occluded pedestrians, those are not labeled for body parts separately. Some researchers also proposed CityPerson dataset as standard for occluded pedestrian \cite{zhang2018occluded}, but as those datasets are not labeled for body parts and labeling dataset is a tedious task, we took an initiative to create a small dataset of human body parts annotation within the full-body images. We have created a data set of human body parts for training our model that consists of 380 images, totaling around 1000 annotations for each different body parts and full body. We have taken 100 images from Penn-Fudan Database \cite{wang2007object}. For testing and evaluating our results, we have created a dataset of 613 images and 622 images of occluded pedestrians.} As some networks like Faster RCNN and SSD-mobilenet can provide satisfactory output with the small dataset we have performed our first training with a small data set. But, training with more body parts data will provide better detection results. We segregate the full body into three parts, namely head, hand, and leg.  We have collected half hand, full hand, a hand with a shoulder, thus covering the most body parts area. We tried to take our data with possible variations, such as taking data from different illuminations (Lights condition, indoor and outdoor as well), occlusion of parts data, and different sizes. Though our dataset is small, we tried to create variation by taking data from different places around the world including India, Bangladesh, Malaysia, Dubai, and the USA.
% We have add some additional raw images from Penn-Fudan Database \cite{wang2007object}, but we have used our own labeling.
\subsection{Training loss}
 %Training: 
\textcolor{blue}{Our training method is the same as the SSD training method, where we need to assign ground truth information to specific default outputs within the defined set of a default output. In the training procedure, our target is to determine the best-matched default boxes within a set of differently scaled bounding boxes for the given ground truth boxes. }
 \todo[inline]{say something related to supervised learning}
We have trained our model with a customized dataset of around 500 images those consists of more than 4000 annotations. We have run our training for around 42000 steps and stopped training after that. 
\todo[inline]{define and explain each loss in Fig. 5}
We showed the change of loss function with the number of steps in Fig. \ref{fig:Loss_function}. From Fig. \ref{fig:Loss_function}, we can see both classification loss and localization losses are gradually declining with the increase of no. of steps. \textcolor{blue}{The red and blue line shows localization loss and classification loss, respectively. The brown line shows the total loss, which is the sum of classification loss and localization loss.} 
\input{figtex/classification.tex}
\subsection{Case studies}
% As we have used the detector for pedestrians from the autonomous cars perspective we checked the result with a video file of pedestrian movement in front of a car. 
\todo{please explain how do you create the video file and what was your setup e.g., by using front-facing monocular camera...}

We have found that while we test the performance of SSD-Mobilenet, there is some false detection with pedestrian crossing signs where those are not actual pedestrians. Another issue is that, in the transition period of body movement, SSD-Mobilenet was unable to detect pedestrians for some of the frames (Figure \ref{fig:Compared result of two model_test_image_2}). On the other hand, While we have tested with our scale specific body parts detection model, for similar types of image frames, our detector can detect some body parts in the transition period and does not confuse by detecting a pedestrian in the pedestrian sign (Figure \ref{fig:Compared result of two model_test_image_2}). Hence, we can say that our model perform better in the case of transitional movement and false detection compared to SSD-mobilenet for particularly pedestrian detection. 
%Comparison results with the transition period are shown in Figure \ref{fig:Compared result of two %model_test_image_1}. 
% \input{figtex/comparison.tex}
% We have to compare different model with our data set and benchmark data set. 
% In analysis we have to describe the strong point of our newly developed model and specifically explained why this model is better than other model.
In our model for creating differently scaled feature maps, we used average pooling. We have tested with some sample images and found that average pooling consists of more information in the contrast region. During the day time, as most of the image has a high background intensity, average pooling performs better as compared to max-pooling. We have taken a sample pedestrian image with average intensity level and found that in the case of max pooling more information is lost as compared to average pooling (Fig. \ref{fig:Result comparison of max pooling_vs_avg_pooling_1}).

\input{figtex/max_pooling.tex}
Fig. \ref{fig:Result comparison of max pooling_vs_avg_pooling_2} shows that with a Max pooling operation, images having high intensity background lost more information compared to average pooling operation. Though max-pooling performed well in the case of a white object with a black background (Fig. \ref{fig:Result comparison of max pooling_vs_avg_pooling_3}), the average pooling result is also satisfactory. So, considering the different intensity levels in the images, average pooling provides more information as compared to max-pooling in the region of changing background intensity. 


\subsection{Performance analysis}
\todo[inline]{
you need to compute followings}
\begin{itemize}
    \item accuracy
    \item precision
    \item recall
    \item F-Score
    \item ROC curve
\end{itemize}
% As we did not find a benchmark dataset for result comparison, we have shown the accuracy of our model with a smaller dataset by checking the no. of objects detected correctly and no. of miss detections.
For analyzing the performance of our trained model we have selected a small dataset of 500 heads, 500 hands, and 470 legs parts and we have found around 93.19\% correct detections for leg, 88.2\% correct detection for hand and 90.8\% correct detection for the head. The correction percentages are pretty satisfactory. We have shown the result in Table \ref{table:Result comparison}. 

\input{figtex/table_result.tex}
We then compare our proposed model with SSD-Mobilenet for 613 image frames of fully visible pedestrians and considering at least one part or full body detection, our model outperforms SSD-Mobilenet model (Table \ref{table:Result comparison of visible dataset} ). 
\input{figtex/table_compare_normal_data_set}
Finally, we compare the performances between our proposed model and SSD-Mobilenet for a fully occluded dataset of 622 image frames and found our proposed model perform significantly better than SSD-Mobilenet for the occluded dataset (Table \ref{table:Result comparison of occluded dataset}).  
\input{figtex/table_dataset.tex}

\subsection{Runtime efficiency}
\todo[inline]{we need runtime comparison and we need to show that our proposed method is faster than SSD-Mobilenet.
}




==> sect/intro.tex <==
Occluded pedestrian detection is a notoriously hard problem in autonomous driving scenarios. For the general pedestrian detection task, we have seen notable progress in computer vision algorithms throughout the last decade. In literature, we also have seen that deep neural networks based detection algorithms typically outperform classical rule-based detection algorithms \cite{zheng2012review, hou2018multispectral, zhao2016faster}. 
For instance, the state-of-the-art algorithm, 
% Deep Feature Pyramid Network (FPN),
SSD-mobilenet,
performs reasonably well in the real-world pedestrian detection problem and significantly better than rule-based approaches \cite{yao2018fully}.

Unfortunately, the occluded pedestrian problem is too challenging for SSD-mobilenet.
% and it appears that the much anticipated improvement in small scale object detection is still an open issue.
% the model used SSD, still has the scope of improvement with very small scale object detection. 
On the other hand, in the real world, occlusion happens very often. Therefore, it is crucial to detect occluded pedestrians using their body parts. Some efforts have been made to handle occlusion in autonomous driving either using a separate module to detect occluded pedestrians \cite{ouyang2013joint} or using a multishot image detector \cite{zhang2018occluded}. However, those methods are not desirable since our main goals for this paper are as follows:
1) to reduce the complexity of the detector and
2) to minimize supplementary computational resources. 

Consider the sudden pedestrian crossing scenario, which has always been a safety issue for autonomous driving. We argue that an autonomous vehicle can avoid such vehicle-pedestrian crashes if it could detect occluded pedestrians in real-time. To do that, given an image frame or a video stream, an occluded pedestrian detection method needs to identify which of a known set of body parts might be present and their corresponding positions within the image frame.

% \todo{explanation of SSD-Mobilenet}
Unlike other object detection methods, the Single Shot Detection (SSD) method takes only one single shot to detect multiple objects in the image frame. We are particularly interested here in the detection of occluded pedestrians with a single image shot. The key idea is to detect at least one body part of occluded pedestrian, which can then be localized in real-time speed.
% \todo{shortcoming of ssd-mobilenet}
In this paper, we have utilized the SSD-mobilenet as our base model. We then proposed a Scale Specific Pooling Model (SSPM), which is developed based on a set of average pooling layers and a set of predefined bounding boxes. We assume that pedestrians who appear too small in the image frame, are located far away from the vehicle. Detecting such pedestrians are not of our interest since they do not violate safety constraints for our application. Hence, we have proposed a set of predefined bounding boxes on top of a feature map to enhance the detection accuracy. Our proposed method is simple and easy to train. In our experiments, we show that our method can learn complex body parts as well as it can detect occluded pedestrians in real-time.


==> sect/prelim.tex <==
% \todo{please write what do you explain in this section.}
In this paper, we have used the SSD-mobilenet as our base model. This model has two parts: Mobilenet \textendash used as the base network for classifying the object types, and SSD \textendash used for localizing the classified objects.

% \subsection{Mobilenet}
Having depth and pointwise separable output Mobilenet creates differs from the traditional convolutional neural networks which do not have separable outputs. 
% \input{figtex/cnn.tex}
Instead, Mobilenet is known as a depthwise separable convolutional network \cite{howard2017mobilenets}, which takes advantage of separable outputs from depthwise and pointwise convolution operations and reduces its complexity compared to other traditional convolutional neural networks. Figure~\ref{fig:Comparison of Convolution}(a) shows symbolic operation of traditional convolution versus depth and pointwise convolution operations  in Figures~\ref{fig:Comparison of Convolution}(b) and Figure~\ref{fig:Comparison of Convolution}(c) that are used in Mobilenet \cite{howard2017mobilenets}. 
\begin{figure}[h!]
    \centering
    \includegraphics[height=3.5cm, width = 8.5cm]{Figures/SSD-Feature_map.pdf}
    \caption{SSD Feature-map operation layers \cite{liu2016ssd}: (a) Input image with ground truth boxes, (b) 8x8 feature map showing default boxes with different aspect ratios those are generated by linearly mapped equation, and (c) 4x4 feature map showing default boxes with different aspect ratios.}
    \label{fig:SSD feature map}
  \end{figure}

% \subsection{Single Shot Detection (SSD)}
% Using the SSD after Mobilenet network, we add an auxiliary structure to the network to detect multi-scale feature maps and default boxes. 
Cascading the SSD with Mobilenet, we can detect multiple objects of different size.
SSD network provides bounding boxes and scores as output. Boxes indicate the location of the object and scores denote the probability of the detected object within the boxes. Training the SSD network with the multi-scale feature map provides the optimum bounding boxes for the detected objects \cite{liu2016ssd}. Figure \ref{fig:SSD feature map} shows the different feature map operation layers of SSD, in which Figure~\ref{fig:SSD feature map}(a) shows the ground truth boxes that are used for training, while Figure \ref{fig:SSD feature map}(b) and \ref{fig:SSD feature map}(c) show the set of default boxes with different feature maps. During the training of an SSD model,  the main goal is to match the default boxes with ground truth boxes \cite{liu2016ssd}. The matching of a default box is calculated using the overall loss function $L$, given in (\ref{loss}), in terms of the localization loss $L_{loc}$ and the confidence loss $L_{conf}$ \cite{liu2016ssd}:

\begin{equation}\label{loss}
    L(x,c,l,g)=(1/N)(L_{conf}(x,c)+\alpha L_{loc}(x,l,g)),
\end{equation}
 \noindent where $N$ is the number of matched default boxes and $\alpha$ is a weight term. The parameter $x$ contains the matching information  in the form of $x_{ij}^p =\{1,0\}$ which denotes whether the $i$\ts{th} default box from the the $p$\ts{th} category matches to the $j$\ts{th} ground truth box. The parameters  \textit{l} and \textit{g} contain the information about the predicted/ground-truth box boxes in the form of $l_{i}^m$ and $g_{i}^m$, where  $i$ refers to the $i$\ts{th} predicted/ground-truth box, and $m\in\{cx,cy, w,h\}$  refers to its parameters, where $c_x$ and $c_y$ are the coordinates of its center, $w$ is its width, and $h$ is its height. The parameter \textit{c} is the multiple class confidence, which contains the information in the form of $c_{i}^p$ which refers to the confidence level of belongings of $i$\ts{th} predicted box to the $p$\ts{th} category. Consider $d_{i}^m$, $m\in\{cx,cy, w,h\}$  a parameter of $i$\ts{th} default box and lets define $\hat{g}$ and $\hat{c}$  as follows:
 
  \begin{equation}\label{ghat}
\begin{split}
	\hat{g}_{j}^{cx} = (g_{j}^{cx} - d_{i}^{cx})/d_{i}^{w},   \hat{g}_{j}^{cy} = (g_{j}^{cy} - d_{i}^{cy})/d_{i}^{h} \\
	\hat{g}_{j}^{w} = log (g_{j}^{w}/d_{i}^{w}), 
	\hat{g}_{j}^{h} = log (g_{j}^{h}/d_{i}^{h})
	\end{split}
\end{equation}

   \begin{equation}\label{chat}
	\hat{c}_{i}^{p} = exp(c_{i}^p)/\sum_p exp(c_i^p)   
\end{equation}

\noindent Then, the localization loss $L_{loc}$ and confidence loss $	L_{conf}$ can be calculated as:

 \begin{equation}\label{loc_loss}
	L_{loc}(x,l,g)= \sum_{i \in Pos}^{N} \sum_{m} x_{ij}^k smooth_{L1} (l_{i}^{m} -\hat{g}_{j}^{m}) 
\end{equation}

\begin{equation}\label{conf_loss}
	L_{conf}(x,c)= - \sum_{i \in Pos}^{N} x_{ij}^{p} log(\hat{c}_{i}^{p}) - \sum_{i \in Neg} log(\hat{c}_{i}^{p})
\end{equation}
\noindent where $Pos$  is the set of indexes for default boxes which contain a detected object, referred to as positive default boxes, and $Neg$ is the set of indexes for default boxes which do not contain a detected object, referred to as negative default boxes.


Having the information about the bounding boxes and scores as outputs of SSD, a non-maximum suppression \cite{rothe2014non} step is used as a post-processing step to produce the final detection, which helps to identify the highest probable object within a single bounding box. 

\begin{figure}[htb]
    \centering
  
    \includegraphics[width=8cm]{Figures/ssd-architecture.pdf}
    

  \caption{Architecture of the SSD-Mobilenet Model \cite{jin2018pooling}.}
  \label{fig:Structure of SSD-Mobilenet Model}
\end{figure}
% Review of part based model if any, address the problem of those methods

% How I am addressing those problem identified in earlier section. 
Figure \ref{fig:Structure of SSD-Mobilenet Model} shows the overall architecture of SSD-Mobilenet. It starts with a MobileNet processing, followed by multi-scale feature maps, which generate bounding boxes and scores as outputs of the network. 
On the development of SSD, Pooling Pyramid Network first introduces the shared tower concept for predicting box score and box location instead of individual box score and box location from differently scaled feature map layers \cite{jin2018pooling}.



%This model has been trained to detect around 90 different types of objects and this model works satisfactorily while it is used for pedestrian detection only. But we found some miss detection in the transition time of pose change. If we trained our proposed model for different body parts, the detector can detect few body parts during the transition time of pose change or movement that enables us to distinguish the performance of the proposed model with the body part detection to full-body detection with SSD-Mobilenet.  
%

==> sect/related.tex <==
% Different Method, Classical, CNN, Pros and cones, why learning is good method: 
Vision-based pedestrian detection can be categorized into two groups:  static pedestrian detection  and dynamic pedestrian detection \cite{zheng2012review}. In this work, we focus on dynamic pedestrian detection, especially occluded pedestrian, using a supervised learning technique.
% \todo[inline]{What kind of pedestrian detection do you propose ... }
\subsection{Classical Methods}
% \textemdash which is a combination of multiple features, and part-based pedestrian detection
% \textemdash which is divided into two groups of model-based and feature-classifier-based),

% \todo[inline]{please Write some glue texts related to classical methods.} Classical method of pedestrian detection or feature based pedestrian detection create a milestone in the development pedestrian detection. One of the major parts of pedestrian detection is feature extraction. 
Classical method can be divided into two groups \textemdash model-based and features-classifier-based pedestrian detection. \todo[inline]{Explain model based detection} .Typically, classical methods employ handcrafted feature extraction to determine pedestrians. Some powerful feature extractors used for pedestrian detection using classical approached are Histogram of Oriented Gradient (HOG)\cite{dalal2005histograms}, Histogram of Oriented Flow (HOF)\cite{dalal2006human}, Scale Invariant Feature Transform (SIFT)\cite{wang2010boosting}, Covariance \cite{paisitkriangkrai2008fast}\cite{tuzel2006region}\cite{gualdi2009covariance}, Haar Wavelet\cite{oren1997pedestrian}, Hierarchical Max (HMAX)\cite{gu2009modified}, and Local Binary Patterns (LBP)\cite{mu2008discriminative}.
% \todo[inline]{Please focus on pedestrian detection problem only, not feature extractions ... }
Although static shape features based pedestrian detection provides a very good platform for pedestrian detection, lacks performance in the scenario of  dynamic shape and varying poses of the pedestrians. Feature-classifier-based detector outperforms the shape model-based pedestrian detectors, but except for the HMAX feature classifiers, all of the other feature classifiers are highly dependent on the large number of training data\cite{zheng2012review}. In \cite{baek2019pedestrian}, combining with binarized normed gradient (BING) method \cite{cheng2014bing}, authors propose the additive kernel support vector
machine (AKSVM) that provides competitive detection speed by generating efficient region proposal. Some researchers combine different features to improve the performance as compared to that of the single feature-based classifiers.
\textcolor{red}{
%In \cite{szarvas2005pedestrian}, a Convolutional Neural Network has been used to detect pedestrians which outperforms detectors with classical feature extractors and classifiers \cite{dalal2005histograms}.
However, classical feature extractors and classifiers for pedestrians detection are not performing satisfactorily in the case of dynamic scenario, occluded pedestrian, and with a different appearance of pedestrians. Hence, we considered a deep learning network to detect occluded pedestrian for the autonomous car.
} 

\todo[inline]{Limitation of handcrafted feature. Please explain the limitation of classical methods and why don't you adopt one of them (from autonomous vehicle point of view)}.

\subsection{Deep Neural Network Based Methods}

% \todo[inline]{please Write some glue texts related to Deep learning.}
Deep learning based pedestrian detection methods have created a milestone by improving performance in pedestrian detection with varies illumination level and complex background with multiple pedestrians. In literature, we have seen convolution neural networks, \textit{e.g.,} R-CNN, Fast-RCNN, Faster R-CNN and SSD-Mobilenet are utilized for pedestrians detection.
To localize an pedestrian in an image, R-CNN \cite{zhang2018occlusion} model combines the \emph{region proposal} method  with CNNs. That region proposal method uses a search algorithm to find candidate regions and then, each region is fed into the CNN network. However, R-CNN model is very slow due to the high computation cost of the search algorithm. To reduce the computation cost, instead of feeding the each region into CNN network separately, Fast-RCNN \cite{girshick2015fast} model feeds the full image  along with the proposed regions resulted from the search algorithm into the CNN network. Faster-RCNN \cite{ren2015faster} implements an improved version of Fast-RCNN by eliminating the search algorithm with a separate network for region proposal. Instead of searching over different regions of an image frame over two steps/networks, Yolo \cite{redmon2016you} uses a single network object detection with the bounding box. 
\subsubsection{Pyramid Network}
Another single network detector has been introduced in \cite{liu2016ssd}, known as Single Shot Multibox Detector (SSD). In SSD, feature maps with different scales, help it to detect different sized objects in a convolutional fashion. Some development on SSD is the Feature Pyramid Network (FPN) \cite{lin2017feature} and Pooling Pyramid Network (PPN) \cite{jin2018pooling}.
% Different Methods for occlusion handling problem, problem of those methods. Why part based occlusion handling method is better. 
Though the different CNN model has created a milestone in object detection, especially in pedestrian detection, a problem like occlusion handling is still a concerning issue which has significant importance for autonomous car and other surveillance systems. Joint Deep Learning model\cite{ouyang2013joint} provides a solution for occlusion handling, but this model is sensitive to localize the pedestrian and slow as, well as this model is not depth-wise separable. Another problem with the deep part model is that this model tried to find out the occluded body parts based on some predefined body structure which is sensitive to pose variation.

\subsubsection{Mobilenet}
SSD-Mobilenet in \cite{howard2017mobilenets} has been prepared for detecting multiple (around 90 different) types of objects. The main challenge with SSD-Mobilenet is that if it is trained for a particular object like a pedestrian, it can not detect pedestrians with some variation of poses, some of the deformed shapes of pedestrians, and partially occluded pedestrians. Besides, if we use SSD-Mobilenet for pedestrian detection, it detects similar types of pedestrian shapes as pedestrian, e.g., it may detects a symbol of pedestrian crossing sign as a pedestrian which creates confusion between real pedestrians and objects similar to a pedestrian. For the steady operation of the autonomous car, it is important to detect the visible parts of the pedestrian if pedestrians' full bodies are not visible. So, we proposed a method for pedestrian detection that can detect pedestrians, along with pedestrians' body parts using the same network.

% \todo[inline]{inspiration of the proposed method and how it works}

Inspired by SSD-Mobilenet and Pooling Pyramid Network (PPN), we proposed a Scale Specific Pooling (SSP) model, which combines a separable network and a shared prediction layer for pedestrian detection.
% \todo{What do you combine?}
One of the major changes in our proposed model compared to SSD-Mobilenet is the replacement of convolution between feature maps with average pooling layers and we have done this differently scaled average pooling based on expected object sizes and ground truth box sizes.


% Organization of the paper. 
% The following section describes the background of the machine vision application for pedestrian detection, then the proposed scale specific model that we have created by tuning some hyperparameters and changing layer sizes for more specific detection is explained. After that, in the discussion section, we show the result that provides better decision-making ability for autonomous cars by detecting body parts of pedestrians in front of the car. Finally, some of the possible areas to improve detector performance have been discussed. 

